Facilitating Exploration with Interaction Snapshots under High Latency

Latency is, unfortunately, a reality when working with large datasets. Guaranteeing imperceptible latency for interactivity is often prohibitively expensive: the application developer may be forced to migrate data processing engines or deal with complex error bounds on samples, and to limit the application to users with high network bandwidth. Instead of relying on the backend, we propose a simple UX design---interaction snapshots. Responses of requests from the interactions are asynchronously loaded in "snapshots". With interaction snapshots, users can interact concurrently while the snapshots load. Our user study participants found it useful not to have to wait for each result and easily navigate to prior snapshots. For latency up to 5 seconds, participants were able to complete extrema, threshold, and trend identification tasks with little negative impact.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> chronicles-infovis-short-2020 (1)/README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> chronicles-infovis-short-2020 (1)/content/abstract.tex <==
Latency is, unfortunately, a reality when working with large data sets. Guaranteeing imperceptible latency for interactivity is often prohibitively expensive: the application developer may be forced to migrate data processing engines or deal with complex error bounds on samples, and to limit the application to users with high network bandwidth.
Instead of relying on the backend, we propose a simple UX design---\emph{interaction snapshots}. Responses of requests from the interactions are asynchronously loaded in ``snapshots''.  With interaction snapshots, users can interact concurrently while the \replace{results load asynchronously}{snapshots load}.
Our user study participants found it useful not to have to wait for each result and \add{easily} navigate to prior snapshots\strikeg{easily}.  \strikeg{We found that }For latency up to 5 seconds, participants were able to complete extrema, threshold, and trend identification tasks with little negative impact.



==> chronicles-infovis-short-2020 (1)/content/ack.tex <==
\add{\textbf{Acknowledgement}: Thanks to Larry Xu for early contributions, Aditya Parameswaran and the anonymous reviewers for their constructive comments. This material is based upon work supported by grants: NSF 1564049 1845638, 1564351, CCF-1730628, OAC-1940175, OAC-1939945, IIS-1452977, DGE-1855886, DARPA D3M (FA8750-17-2-0107), and DOE DE-SC0016934, as well as gifts from Alibaba, Amazon Web Services, Ant Financial, CapitalOne, Ericsson, Facebook, Futurewei, Google, Intel, Microsoft, Nvidia, Scotiabank, Splunk and VMware.}


==> chronicles-infovis-short-2020 (1)/content/conclusion.tex <==
\section{The Interaction Snapshot Design Process}

% ew
Having presented \replace{ways to create snapshots of interactions by example}{examples of interaction snapshots}, we now conclude with a generalized design process. Interaction snapshots  require three elements: (1) the user's past interactions, (2) the effect of each interaction, and (3) the temporal ordering of the interactions.
\replace{These three components }{Together, they} show the correspondence between the user's interaction \add{requests} and the response of the system over time.
There are different ways to satisfy these requirements. 
For the \strikeg{pilot }bar chart, we used \replace{Bertin's ``position'' visual}{the position encoding} channel\add{, which can be applied to other single visualizations.}\strikeg{, and }
For the dashboard, we used \replace{thumbnails}{snapshots}\add{, which can be applied to other multiple coordinated visualizations}. 
\strikeg{These two designs in fact generalize to most common interactions---either single chart interactive visualizations or multiple coordinated visualizations.}
% However, there may be other techniques for creating interaction snapshots.

% point to interesting things we need to study
Through many pilots and design iterations, we explored aspects of the design space for multiple concurrent interactions.  We found a positive answer to our initial question of whether frontend design alone could offer some alleviation to the pain of latency.
We have also opened up new questions.  One idea is to more systematically study how snapshots change user behavior in terms of rates of observations, drawing generalization, and forming hypothesis\add{, following prior work}~\cite{liu2014effects}\replace{.  We could also}{ and} compare interaction snapshots and progressive/optimistic visualizations.
Another idea is to further develop controls around the snapshots\replace{---participants voiced interest\strikeg{s} in}{such as} editing and organizing\strikeg{ the snapshots}.  \add{We could also augment the linear history with when users ``branched'' off into a different interaction to capture richer context---the snapshots could double as an interaction provenance graph.}
More broadly, \emph{interaction snapshots} present\strikeg{s} opportunities to bring features common in literate computing to interactive visualizations\strikeg{that are usually transient}.

% Interaction snapshots contribute one alternative design to the world of big data visual analysis.

==> chronicles-infovis-short-2020 (1)/content/evaluation.tex <==
\section{Dashboard Snapshots: Design and Evaluation}

The pilots evaluated interaction snapshots' effectiveness on a single visualization for fixed tasks.  We now evaluate the technique for a more complex setting---dashboard---with open ended exploration.

One key design challenge with snapshots for dashboard is \emph{space}.  Replicating the interaction results as small multiples is not feasible for dashboards.  We address this constraint by creating a separate representation of the snapshot---a smaller ``thumbnail'' view, much like Graphical Histories~\cite{heer2008graphical} and Pangloss~\cite{moritz2017trust}, which can be clicked on and expanded. 
% An example is shown in 
Figure~\ref{fig:demo} is an example application of the technique on a cross-filter visualization of wildfires in the US~\cite{fires}.
% say something about how they can make interactions without waiting
\add{The interaction details and code are included in supplementary materials.}

%%%%%%%%%%%
\subsection{Methods}

Rather than assigning participants specific tasks (as in previous pilots), we \strikeg{plan to }observe how participants explore data and \replace{use more}{report} qualitative metrics.  First is whether and how much the \replace{analysts}{participants} make use of concurrent multiple interactions.  A higher usage would suggest that the snapshots design is able to facilitate concurrent interactions, and that it is useful to the participants.
Second is how often snapshots are revisited\replace{.  Since traditional dashboards reduce to the most recent snapshot, }{---}the more participants engage in older snapshots, the more they are leveraging interaction snapshots' unique capabilities.
Third is direct feedback.

We conducted a first-use study with 6 \strikeg{representative }users, all college students who have taken data science courses, with a self-reported ``somewhat experienced'' with visual data analysis on a 5-point Likert scale $(\mu=3.0, \sigma=0.89)$.
Due to the COVID-19 ``shelter-in-place'' order, we conducted the studies over video.
We began each study with a 5-minute tutorial of the interaction snapshot enabled dashboard on mass mobilization protest data~\cite{DVNHTTWYL2016}, and then asked participants to \replace{analysis}{analyze} US \replace{wild fires}{wildfires} using a similar dashboard (Fig.~\ref{fig:demo}).
Participants \replace{are}{were} \replace{promoted}{prompted} with a specific question (``identify the states with the most \strikeg{number of }wildfires in the years 2000 to 2004'') followed by free-form exploration for about 8 minutes. \replace{At the end}{Then}, participants verbally summarize\add{d} their findings.
All interaction latency \replace{is}{was} set to between 5 to 7 seconds.
At the conclusion of the study, we administered an exit survey to measure the effectiveness of the interface and to debrief participants about their experiences.
The \strikeg{whole }session took 20-25 min and participants were compensated \strikeg{with }\$15 in Amazon gift cards.

%%%%%%%%%%%%%%%%%%
\subsection{Quantitative Results}

We instrumented the interface to log all user interactions, including interactive selections of elements in the charts, navigating to prior interaction states, and scrolling through the snapshots.
To analyze this data, we visualized the traces in Fig.~\ref{fig:eval_trace}.  For the interactions that happened \emph{before} the previous interaction was loaded (since there is a 5 to 7 second delay), we mark them as \emph{concurrent interactions} (\textcolor[HTML]{0868ac}{\smc{concInteract}}, as labeled in the Chart)
% \remco{is there somewhere (either here or in the section before) where you can make a statement or two that makes it clear that we consider ``more'' concurrent interactions to be ``better'' (and remind the reader as to why)?}, 
% Yifan: ok I'll add this to the methods/hypothesis section
the rest of the interactions as \textcolor[HTML]{239023}{\smc{interact}}.  We also provide a distribution of the percent of concurrent interactions out of all interactions in the bar chart to the right, with ($\mu=0.38, \sigma=0.10$).  Participants interacted with the interface on average 20 times $(\mu=20.33, \sigma=5.99)$ during the session, and navigated twice that \add{on }average $(\mu=43.17, \sigma=17.49)$.

% \subsubsection{Post-study survey results}

On 5-point Likert scales, participants positively rated the interface overall $(\mu=4.33, \sigma=0.47)$, as well as the history feature $(\mu=4.17, \sigma=0.69)$.  In terms of how frustrating the delay was, participants rated it as only a little $(\mu=2.0, \sigma=0.58)$.

% When asked ``How was your overall experience with using the interactive visualization?", participants answered on average that it is ``Good'', on a Likert scale from ``Very poor'' to ``Very good''.  When asked ``How did you find the history feature (thumbnails)?'', participants answered on average that it is ``Helpful'' , on a Likert scale from ``Very unhelpful'' to ``Very helpful''. Lastly, when asked ``Were you frustrated with the delay in data processing (red spinners)?'', participants answered ``Little''  on a Likert scale from ``Never'' to ``A great deal''.
% summarize visualizes the traces of As visualized in , All the participants engaged with the history by clicking on thumbnails or using the arrow keys to navigate.
% describe ways in which they engaged with history
% first is concurrency

%%%%%%%%%%%%%%%%%%
\subsection{Qualitative Results}

We observed participants quickly grasped how to make use of concurrent interactions through the snapshots.
% All the participants used concurrent interactions, though to varying degrees.  .
% qualitative
% people liked concurrent interaction
One common pattern was to make multiple interactions concurrently when the participants had a question in mind.  P3 mentioned that it was ``\textit{nice to have [the interaction result] pre-loaded}'', and that reminded them of ``\textit{opening search results in multiple tabs [in the background] when browsing web pages}.''  P6 also indirectly commented that ``\textit{Tabs [i.e., snapshots] made the wait less painful/annoying.}''

However concurrent interactions are not always used. When participants had a specific question or targets in mind, such as ``I want to compare how different causes of fires differ geographically'', they knew exactly what interactions they would need and opted for concurrent interactions.  When the participants did not have such a question, they relied on the results to their immediate selections to generate ideas for further interactions. Hence they waited for the response to load instead of making other interactions while waiting. 
% \remco{awkward sentence}.
% another
Interestingly, the snapshots still proved useful while they \emph{waited}.  P4 mentioned that when they were waiting for the result to load, they would ``\textit{look at the history to remember what I was doing earlier to keep track of what I'm looking for}''.  P1 also used the delay to positive effect, saying that ``\textit{the delay gives my brain a time to reflect on what I'm expecting and what to do. I think it's actually better [than instantaneous response]}.''  None of the participants found the delay to be more than a little frustrating.


All of the participants \replace{used navigation}{browsed} through history when summarizing their findings\replace{.  For the final task of summarizing findings, they browsed through history}{ (the final task)}, recalling relevant insights they made prior.  This can be seen in the dense patches of \textcolor[HTML]{d95f0e}{\smc{navigate}} ticks towards the end of the sessions in Fig.~\ref{fig:eval_trace}.
P6 mentioned that ``\textit{History tool allowed me to go back to my previous thoughts easily, and made it easy to reference observations.}''

% people had more feature requests.
\strikeg{However, }Participants also desired more features.  P4 mentioned that the snapshots quickly became visually cluttered and difficult to navigate, which detracted from the positive aspects of history.
P3 suggested ways to introduce more guides for the snapshots, such as adding text to describe \strikeg{what }the interaction \strikeg{was}, or a way to either arrange or color encode the snapshots by the chart interacted with.
\strikeg{Both }P3 and P4 asked about the ability to remove snapshots that they found irrelevant.


==> chronicles-infovis-short-2020 (1)/content/intro.tex <==
% latency is reality
Current interactive data visualization systems rely on fast response times to provide a good user experience.
This approach simplifies the design of the visualization UI and ensures direct manipulation interfaces that facilitate fluid user data exploration~\cite{liu2014effects}.  However, interactive data visualization is increasingly an integral part of big data analysis.  The scale of the datasets and the required computational power has made it necessary to shift the data processing and storage to remote data\add{bases}\strike{management systems}.  In such a client-server architecture, client interactions are translated into server requests that incur both data processing and network latency.
Ensuring ultra fast response times in the face of all these latencies is often challenging if not impossible.  The interface therefore should have a backup plan should the latency be high---the frontend needs to be resilient to high latencies.
% , while the backend try to reduce the latency,

Prior work, such as progressive visualization~\cite{hellerstein1999interactive, fisher2012trust, zgraggen2016progressive, fekete2016progressive, rahman2017ve} and optimistic visualization~\cite{moritz2017trust}, have also utilized interface design to deal with latency.  However, these approaches still rely on considerable backend instrumentation, namely online aggregation~\cite{hellerstein1997online, hellerstein1999interactive, kraska2018northstar} and approximate query processing~\cite{ding2016sample, agarwal2013blinkdb}.
% ew
\add{In many settings, designers do not have the opportunity, desire, or resources to make changes to the backend database systems.}

% P4: bluntly state that the state of everything is single (make it weaker), 
% ew
\replace{Critically, all these approaches focus on 
how to address}{Current UX-oriented solutions primarily address} usability challenges stemming from a \emph{single} user request.  They focus on ways to shorten the time between the frontend sending the request to the backend and receiving the response.  For instance, progressive visualization updates a single selected visualization with more accurate results over time.
% ew
\replace{When the user want\add{s} to make another interaction while the previous is still being processed, the vast majority of existing designs only allow one interaction to be handled at a time\add{ (with the exception of optimistic visualization, which we discuss in Section~\ref{sec:related})}.
We \add{now} discuss the two most common designs.}{But what happens when the user wishes to make another interaction while the previous is still being processed? We now discuss the two predominant designs.}
% limit the number of outgoing request to one.
% which will send a different request to the backend
% We now describe what these common designs are and highlight the missing opportunity to rethink how multiple requests could be handled.

One such design is ``blocking'', where users are not allowed to perform a new interaction until the prior ones have rendered.  This design makes the most sense when the latency is negligible, which is often the case when the data is small and fits in memory, such as the case for Vega~\cite{satyanarayan2015reactive} which runs on the browser, and Excel.  The design is easy to implement and puts the least amount of load on the backend.  As a result, even client-server systems like Tableau, which may not always guarantee negligible latency, adopt it.

Another common design is to allow new requests to be made and cancel previous requests.  Allowing the user to interrupt existing requests makes the interface more \emph{responsive{\strikeg{ness}}} and ensures that ``time-consuming operations that block other activity'' can be aborted~\cite{johnson2007gui}.  The interface \strikeg{will }render\add{s} the results of the most recent interaction\strikeg{s} only.

% talk about what happens if they do NOT cancel.
If the previous interaction is \emph{not} cancelled, then more than one pending request will be processed concurrently, which has potential to reduce the overall latency and improve user experience.
However, rendering interaction responses concurrently runs contrary to \textit{direct manipulation}\cite{shneiderman1982future, hutchins1985direct}, a commonly held user-interface design principle.
% .  As shown by Hutchins et al. , there are cognitive benefits to a direct manipulation interface because it reduces the \textit{semantic} and \textit{articulatory} distances between the user's actions and goals.
Direct manipulation requires that ``the object of interest is immediately visible'', which in effect assumes a serial relationship between a user's action and the system's response in a one-to-one fashion.
In contrast, allowing multiple responses to render concurrently behaves in an opposite manner---when a user interacts with a number of visual elements, the system might not respond to these interactions in the sequence the user's actions are performed or to replace the results too quickly. Both of which can be confusing to users by making it difficult to reason about the \emph{correspondence} between interaction and response and to make sense of the responses.

\begin{figure}[b!]
  \centering
  \includegraphics[width=\columnwidth]{figs/fires_demo.png}
  \caption{Applying interaction snapshots to a cross-filter visualization. Evaluation of US \replace{wild fire}{wildfire} data.  As users interact, snapshots are created.  Users can perform \replace{``concurrent''}{\emph{concurrent}} interactions where they do not have to wait until the previous results arrive.}
  \label{fig:demo}
\end{figure}

% when the results are flashing/out of odrer, hard to reason about the correspondence between interaction and response. We hypothesize that this is taxing, and visualizing these relationshipships explicitly can be benefitial. 
% ack comes at a cost of space and needs user
To harness the benefit of concurrent interactions, we must address the design challenge it imposes.  Our approach is to visualize the coordination between asynchronous request and responses explicitly.  We do so by capturing the interaction results in a sequence of \emph{snapshots}.  This way, each new result of an interaction is appended to a history of results. Snapshots provide a stable frame of reference that helps users make sense of uncertain latencies.
% While latencies may be non-deterministic, the order of interactions made by the users are.
Given this easy visual reference, the users could view the snapshots at a later time once the response is received.
Snapshots mediate the asynchronous results through history and create a direct manipulation experience for multiple concurrent interactions.

Consider a cross-filter application, as shown in Fig.\ref{fig:demo}.  After a user makes an interaction, a snapshot is created and appended beneath the visualization dashboard.  The snapshot is a scaled-down display of the current visualization which continues to load while other snapshots are appended.
The snapshot gives a visual indicator (e.g., spinner) of whether the data is still being processed.  When the user sees the visual indication that the processing is complete, they can click on the corresponding snapshot, which loads the processed visualization into the main view for analysis.
Users can also navigate through the snapshots quickly with left and right arrows, which ``animates'' through the selections.

% talk about some of the nuances of this interface
We evaluated the efficacy of interaction snapshots on dashboards with 6 participants. Traces of participant behavior demonstrate they can make effective use of concurrent interactions and navigate to different snapshots.  Qualitative feedback reveals that participants find the interaction snapshot design helpful in the face of latency.

% engaged in concurrent interactions and navigated between snapshots.  Overall, they

% here for awk layout problems
% \begin{table*}[t!]
%   \begin{center}
%     \begin{tabular}{|p{2cm}|p{9cm}|p{4cm}|}
%     \hline  & \textbf{Backend Methods} & \textbf{Frontend Designs} \\ \hline
%      \textbf{Deterministic} & GPU-based compute~\cite{liu2013immens, mapd, graphistry}, custom indices~\cite{lins2013nanocubes, tao2019kyrix} & interaction snapshots \\ \hline
%      \textbf{Probabilistic} & Approximate query processing~\cite{agarwal2013blinkdb}, online aggregation~\cite{hellerstein1997online}, progressive visualizations~\cite{fisher2012trust, zgraggen2016progressive, fekete2016progressive},  intelligent prefetching of data ~\cite{battle2016, moritz2019falcon} & optimistic visualizations~\cite{moritz2017trust}\\\hline
%     \end{tabular}
%     \label{tab:related}
%   \end{center}
% \end{table*}


==> chronicles-infovis-short-2020 (1)/content/pilot.tex <==
\section{Design Iterations}

\begin{figure}[tb]
   \centering
   \includegraphics[width=0.8\columnwidth]{figs/events.pdf}
   \caption{A sequence of interaction requests and responses under different conditions visualized on a horizontal time axis.  Colored arrows represent request/response pairs over time. Light vertical lines highlight request times. Case (1) is the ideal no-latency scenario commonly assumed by visualization designers---everything works as expected.  (2) With latency, the user waits for each response to load before interacting.  (3) With latency, the user interacts without waiting, and in-flight responses are not rendered.  (4) With latency, the user interacts without waiting, and all responses are rendered.  (5) With latency, the user interacts without waiting and may see responses in a different order than requests were issued.}
   \label{fig:events}
\end{figure}

% do a quick discussion on what we are dealing with
To design with latency, we first analyze different ways interactions are handled in the presence of latency.
The top diagram in \replace{Figure}{Fig.}~\ref{fig:events} depicts a time-ordered model, where time increases from left to right. User inputs are depicted along the top line (interaction history), and the responses are rendered along the bottom line (render history). A dashed arrow between the interaction and render history corresponds to the time to respond to the request.


\begin{figure}[b]
   \centering
   \includegraphics[width=\columnwidth]{figs/pilot1.png}
   \caption{Pilot experiment: on the left is the basic design where interaction results update in place, on the right is a design that displays snapshots of interaction results as small multiples.}
   \label{fig:pilot}
\end{figure}


\begin{figure}[tb]
   \centering
     \includegraphics[width=0.7\columnwidth]{figs/pilot_time.pdf}
   \caption{Comparison of median users task completion times, with the \emph{interaction snapshots} condition being much faster than the others.}
   \label{fig:pilot_time}
\end{figure}

\replace{Figure}{Fig.}~\ref{fig:events}(1) shows the ideal case where requests respond instantaneously. However, \replace{assuming}{when} there is latency\strike{ in the system}, a number of possible scenarios can occur: \strikeg{For example, }(2) shows the blocking case where the user is not allowed to submit a new request until the prior one\replace{ is rendered}{completes}; (3) shows the non-blocking case where users freely interact with the visualization and new requests supersede and cancel previous requests; (4) \replace{illustrates}{shows} the concurrent case where neither the input nor the output is blocked. The benefit of this approach is that the total time is shorter, but the downside is that the interface could be difficult to interpret, especially when the amount of latency varies\strikeg{, as shown in } (5).

\begin{figure}[tb]
   \centering
     \includegraphics[width=0.7\columnwidth]{figs/concurrency_time_scatter_longdelay.pdf}
   \caption{Completion time correlated with level of concurrency. A negative correlation suggests that concurrent interactions may help alleviate the effect of latency.}
   \label{fig:pilot_concurrency}
    %   ---the percentage of task completion time where there was more than one concurrent request
\end{figure}

\begin{figure}[tb]
   \centering
   \includegraphics[width=0.75\columnwidth]{figs/exp2_all_edit.pdf}
   \caption{Each chart of the plot visualizes median task completion time with 95\% CI (y-axis).}
   \label{fig:exp2_all}
\end{figure}



To address the dis-coordination between interaction request and response, as seen in \replace{Figure}{Fig.}~\ref{fig:events}(4,5), we hypothesize that displaying past interactions in snapshots could serve as a stabilizing visual anchor.  
% \jmh{how about a graphic kind of like Fig 2 but with the synchronous creation of thumbnail as a level of indirection. "Put a pin in it"}
% I'm going to discuss it as a technique.
A simple mechanism is to encode the step by which the interaction was made using a\strikeg{n additional} visual encoding channel.  The right of Fig.~\ref{fig:pilot} shows an example where \strikeg{snapshots of month }selections are rendered \add{in snapshots}.
% as small multiples.
% we used position to encode the history and results of interactions (from clicking month buttons). 

We conducted a pilot study to verify the hypothesis.  In the pilot, participants used a simple visualization shown in Fig.~\ref{fig:pilot}: a bar chart that displays sales data for a company across years, split into facets of the months.
There are three conditions: baseline, treatment 1 and treatment 2. The first two uses the interfaces on the left of Fig.~\ref{fig:pilot}, and the last one the right of Fig.\ref{fig:pilot}.
The baseline is the blocking interaction, as illustrated in Fig.\ref{fig:events}(2). Treatment 1 has the same UI as baseline, but asynchronously renders the results, as in Fig.\ref{fig:events}(4,5).
Treatment condition 2 shows interaction snapshots.

Participants were asked to identify if any of the months crossed the sales threshold of $80$ units sold. 
% We generated data to ensure the task was not perceptually difficult.  There were no data points that were close to the threshold of $80$ units. 
% 50\% of the assignments exposed to a user had exactly one month above the threshold, and the other 50\% had no months above the threshold 
% \remco{this part is a little confusing. It took me a couple of reads to realize that the data is randomly generated or that there are two datasets}. 
We measured the accuracy of the response and the total time to complete a task in seconds \add{(the time between when the participant is allowed to start interacting and when the they submits an answer)}.  We also logged all events on the UI, such as \strikeg{hover }interactions, responses received, and response rendered.

% We chose a very simple visualization and task because if we cannot elicit concurrent interactions in a simple setting, it would be even less likely in a complex interface.  Furthermore, this hover-response visualization is similar to cross-filtering and brushing-and-linking visualizations.

We recruited participants online through Amazon Mechanical Turk (17 participants for baseline, and 30 for the two treatments, 58\% with bachelors degree or higher, and 46\% female, ranging from 23 to 67 years of age).  \add{Participants were compensated \$0.30 per task, with a \$3-5 completion bonus, compliant with Californian minimum wage.} Participants were randomly sorted into either the baseline or treatment group.  They were shown instructions about the task and trained to complete two sample \replace{assignments before completing actual assignments}{tasks beforehand}.

The differences were in task completion time, shown in Fig.~\ref{fig:pilot_time}.  We report the unsigned Wilcoxon Rank-Sum test: baseline median=37 sec (N = 31), treatment (condition 1) without snapshots median=33 sec (N=52), Z=0.63, $p<0.5$, and treatment (condition 2) with snapshots median=17 sec (N=54), Z=3.22, $p<0.002$ where N denotes the count of the group.  There were no significant \strikeg{accuracy }differences \add{in accuracy} between the three conditions.  \add{We can see that participants were able to complete the tasks much faster with the snapshots design.  To understand why this was the case, we visualized the concurrency---the percentage of task completion time where there was more than one concurrent request. Fig.~\ref{fig:pilot_concurrency} show that participants \strikeg{could complete tasks faster }with higher concurrency\add{ tend to complete tasks faster}, which is made possible because of asynchrony and encouraged by the snapshot design.}

% now talk about generalizing the tasks
% \remco{this sounds like a different pilot. Should present it as such} 
To ensure that the result also generalizes to other tasks, we conducted a second pilot study to include two more tasks: identifying the month with a maximum value, and the month with a certain trend. These two tasks represent the ``find maximum/extremum'' and ``characterize distribution'' tasks in Amar et al.'s analytic activity taxonomy \cite{amar2005low}. Both of these tasks are known to be more challenging than the threshold task in the first pilot study, which falls under ``retrieve value'' in the taxonomy.  Each participant completed the tasks with either no snapshots (baseline) or with snapshots designs (treatment).  We also have two latency conditions: one is uniformly sampled from 0 to 1 second (short), and the other is  uniformly sampled between 0 to 5 seconds (long).  Each participant completes three conditions (none, short, and long).  For each group, we recruited 50 Mechanical Turk participants.  Again, we found that there were no significant differences in task accuracy.  Task completion time, however, was very different, as shown in Fig.~\ref{fig:exp2_all}.  We see that participants complete all tasks significantly faster in the with-snapshots condition when there was \add{long} latency. 
% \remco{what is the right most chart in Figure 6? (named ``Threshold'')}


% \begin{figure}[tb]
%   \centering
%   \includegraphics[width=0.75\columnwidth]{figs/exp2_concurrency_regression_task.pdf}
%   \caption{A scatter plot of accurately completed tasks' completion time against concurrency, faceted by tasks, under high latency.  Pearson's $r$: threshold $r =-0.60, p<0.00001$, extrema $r = -0.60, p <0.00001$, and trend  $r =-0.50, p<0.00001$.}
%   \label{fig:exp2_concurrency}
% \end{figure}

% subjective reporting
% TODO: say something more about how the ease of use is more important than just saving some seconds.
More qualitatively, participants commented that completing the tasks with latency with no snapshots is ``painful'', ``frustrating'', ``tedious'', and ``awful''.  Some explained that responses were hard to remember---\emph{``I had a hard time remembering what I'd just seen a second ago.''}.
In contrast, participants commented on the ease of use when snapshots are present---\emph{``The ability to load several months at once definitely offsets any loading latency -- difficulty was roughly the same as one month with no latency. One month with latency was a bit painful.''}.  Interestingly, the perceived speed of loading seemed to have changed as well---\emph{``Some of the tasks loaded really slow, single month got irritating waiting.  Most of the multiple tasks loaded fairly quickly.''} While the perception of latency is not the focus of this study, \replace{such participant}{the} feedback suggests the benefits of the use of \replace{``interaction snapshots''}{interaction snapshots} beyond improving \strikeg{the participants' }task-completion times~\cite{harrison2007rethinking}. 
% \strike{For instance, how progress bars progress changes how people perceive the speed ~\cite{harrison2007rethinking}.} 

\begin{figure*}[tb]
  \centering
  \includegraphics[width=\textwidth]{figs/eval_event_trace.png}
  \caption{On the left is a visualization participants' interaction traces while exploring  US \replace{wild fire}{wildfire} data. The traces visualized are interactions---which contains both concurrent interactions (\smc{concInteract}), and non-concurrent interactions (\smc{interact}).  On the right is the percent of concurrent interactions of all interactions made.}
  \label{fig:eval_trace}
\end{figure*}


% took some getting used to, and slows down
\replace{Snapshots}{The interaction snapshots design} was not free from fault. One participant commented that ``It took a few tries to get used to how it worked''.  We also see evidence of this in \add{Fig.~\ref{fig:exp2_all}---under} \strikeg{the results for }the no-latency condition, \strikeg{where }participants took on average \strikeg{slightly }longer to complete \strikeg{the maximum }task\add{s} when using the new design compared to baseline.

==> chronicles-infovis-short-2020 (1)/content/related.tex <==
\section{Related Work}
\label{sec:related}

\noindent{\textbf{Dealing with Interactive Latency:}} Prior work addressing the issue of latency in interactive visualizations can be divided along two axes: whether the solution is provided by the backend or the frontend, and whether the query is evaluated on whole or samples of the data.

% . One is whether the solution involves front-end design changes, and another is whether the solution is deterministic or
Backend techniques to reduce latency for queries over all of the data include GPU-based compute~\cite{liu2013immens, mapd, graphistry}, custom indices~\cite{lins2013nanocubes, tao2019kyrix}, and prefetching~\cite{moritz2019falcon, battle2016}.
Backend techniques for a probabilistic query trade some amount of uncertainty for the reduction in processing time.  These include approximate query processing~\cite{agarwal2013blinkdb, ding2016sample} and online aggregation engines~\cite{hellerstein1997online, hellerstein1999interactive} from which \emph{progressive visualization}~\cite{hellerstein1997online, fisher2012trust, zgraggen2016progressive, fekete2016progressive, rahman2017ve}, which we discuss in the next paragraph, is based on.
% , online aggregation~\cite{}.  
% There are also algorithms to predict future interaction targets to prefetch relevant information, which could be non-deterministic.
While innovations in these backend techniques improve computation capabilities, they do not eliminate the existence of latency in the real world.  Users could be dealing with legacy systems, large amounts of data, or, sometimes, slow network connection.

Compared to the pure backend efforts, our work is more closely related to progressive visualization, which \strikeg{develops around the idea of }\replace{streaming}{streams} partial results (containing error bounds) to users.
\add{An augmentation to the streaming design}
\strikeg{Another related idea} is  Moritz et al.'s \emph{optimistic visualization}, which allows the user to first interact with an approximate query engine, and lets users mark an interaction as ``remembered'' for a full, non-approximate, evaluation to check later~\cite{moritz2017trust}.

We take inspiration from these work's approach of leveraging design to adapt to the realities of ``big data''. 
\add{In particular, optimistic visualization allows for users to optimize \emph{across} interactions, from which our design builds on.}
However, both progressive and optimistic visualization rely on approximate query processing.
Since on-the-fly sampling cannot cover every small subset of data, many approximate query techniques also involve precomputing samples, sketches, or other summary structures~\cite{cormode2012synopses}. The preprocessing steps require time, computation, and storage for each precomputed result.
\add{The additional effort may be worthwhile for developers who could afford backend changes, e.g., adapting advanced engines like \emph{Sample+Seek}.  For those who would rather make changes just to the frontend, interaction snapshots may be a more preferable trade-off---developers just need to add the new UX technique and potentially limit their interaction designs to avoid ones that would trigger a large amount of interactions, such as continuous brushing.}
\strikeg{Interaction snapshots, as a simple UX technique, does not depend on these more involved backend efforts.}
% \add{Snapshots may also require developers to avoid .}
% \subsection{Interaction History}

\medskip
\noindent{\textbf{Interaction History:}}
Much prior HCI work has used interaction histories to facilitate user actions.  
Work in the CSCW community used trails of cursor positions to give temporal context to the actions of remote participants~\cite{savery2011s}.
In the visualization community, Heer et al. model history as a sequence of movements through a graph of application states, presented in thumbnails in \emph{Graphical histories}~\cite{heer2008graphical}.
Feng et al. externalized interaction history by showing the ``footprints" of interactions\cite{feng2017hindsight}. Optimistic visualization, as mentioned earlier, also makes use of history (the ``remember'' feature) to help users verify approximate results~\cite{moritz2017trust}.

These prior work inform our design.  Feng et al. observed that a direct encoding of interaction history supports visual recognition of previous interactions. The visual history does not require users to recall the past, which can be mentally taxing.  The observation inspired us to visualize interaction history to reduce the cognitive challenges to asynchronous interactions.  Graphical histories gave us inspirations for how to design the snapshot for dashboards, and optimistic visualization gives initial support that users do revisit interaction history when exploring data.


==> chronicles-infovis-short-2020 (1)/content/scrap/design_scrap.tex <==

% show that presenting interaction histories do indeed facilitate users performing concurrent interactions when confronted with latency.  
% \remco{separate this sentence into two. First state what the generalized design is for? (e.g. ``We now present the generalized design for using interaction histories to XXXX.'' Then, the second sentence will be something like ``Named ``Chronicles'', this design requires three elements...''}: 

==> chronicles-infovis-short-2020 (1)/content/scrap/eval_scrap.tex <==
% \remco{need a conclusion section here... It's possible that 5.2 becomes the conclusion section? Not sure... but it feels weird to have a paper without one.}

% also just context
% History also proved useful outside of the context of concurrent interactions---it aided .  , all the participants clicked on a subset of past thumbnails, using the visuals as a base to recall their findings.


% The reason why not all interactions are concurrent can be explained by the analysis activities.  When participants had a specific question that compares across interactions, such as comparing between the fire counts by state across the years, they would concurrently specify their interactions. 

% A major limitation of Chronicle's approach is that it would only work for interactions that are not dependent on the previous interaction. Take Figure~\ref{fig:demo} as an example, if the analyst wishes to drill into states where the carrier United has the highest count of flights, then they necessarily have to wait until the data is loaded \jmh{for per-state carrier rankings} before they can proceed with the interaction \jmh{on the chosen states}.
% \jmh{Fig 1 is too small to understand at this level of detail.}
% However, as we have demonstrated in the pilot studies, there are basic tasks that involve interactions that are known ahead of time, such as finding a maximum, identifying if a threshold is crossed, identifying trends across interactions.  
% Furthermore, even for the aforementioned task where the next step is dependent on the previous, the user may benefit from having immediate access to the visualization state earlier in case they do not remember all the relevant values from some latency ago.

% The cases where one interaction may depend on a previous interaction state, as is the case of cross-filter, also uncovers possible extensions to the simple linear history we presented.  Future designs could iterate on a more complex tree-like thumbnail design that is shown on demand.

% Lastly, we need to conduct further user studies with more advanced tasks such as free form data exploration.  We also need to compare with progressive visualizations to get a better understanding of how the approaches compare.


% however, even if Chronicles cannot alleviate all the effects of delays, it is still valuable.



% talk about the different times when they do concurrent and when they don't---when they have a specific question to compare, they do, when they do not know what they are looking for, they need the result to inform their next steps.



% point toward literate computing

% Say that what we find with history corroborates with Moritz et al's finding "we might also group visualizations in the history by their broad tasks." --- say something along the lines of literate computing, the duality of seeing interactions as requests and in gneral artifacts that can be further worked with.





% talk about limitations, such as how we were not able to compare this against progressive visualizations.

==> chronicles-infovis-short-2020 (1)/content/scrap/future_scrap.tex <==

% that capturing interaction history in snapshots encourages users to make better use of waiting time. 

% To conclude, we discuss he last user study reveals opportunities for 



% open up the realization about history

% make it like a continuation of work that leverages interaction history
% By aiming to support concurrent interactions, we (re)discovered the power of history.  We could explore different affordances for the thumbnail design.

% TODO
% \jmh{I found this paragraph confusing and eventually unsatisfying once I unpacked it. It says that you have to wait on (cannot parallelize) data dependencies.  E.g. if you have two expressions $z = g(y)$ and $y = f(x)$, you have to wait for $y$ to be computed before you can execute $g(y)$. This is not a limitation of Chronicles per se. It's also weird to say "but there are cases where you don't have data dependencies." Of course there are. So question to you: if this is a "limitation", (a) what do you propose to do about it, and (b) how big of a limitation do you want to say it is? My personally feeling is that it's not a limitation of your work at all, it's an orthogonal fact about the real world that you can't do $g(f(x))$ before you do $f(x)$ and nobody would ever try to do so!!}


% Beyond assisting the analyst with tools against high latency, we hypothesize that the visual history may help analysts recall past insights and construct a narrative.
% In addition, the exact design of the history merits further design iterations---how long of the past should we show? Should we give users a way to store a view for future comparison manually?


==> chronicles-infovis-short-2020 (1)/content/scrap/related_scrap.tex <==

% Instead of progressively loading more data per interaction, we progressively load more results over a sequence of interactions. , but unlike Pangloss, interaction snapshots uses it as a stablizing frame of reference for asynchronous visualizations.
% The design space for asynchronous is orthogonal to progressive visualizations and face different trade offs.
% As a result, the challenges of the interface are also different. 

% Progressive visualization requires users to interpret uncertainty, whereas interaction snapshots requires users to specify interactions in advance of seeing previous results.
% diff
% Given that they lie in different design spaces, the two techniques are not mutually exclusive\,---\,design could compose Chronicles with progressive visualization to further enrich mechanisms against latency.


% Both progressive and optimistic visualizations need to work with sampling.  



% We now discuss in more detail how our approach relates to progressive and optimistic visualizations, both of which do make use of front-end design changes.

% We will not provide a detail discussion for backend methods to eliminate latency since our solution is concerned only with interaction design.  Our audience is those who have to work with some latencies, much like the audience of the progressive visualization research.  We will also discuss other research that make use of interaction history and how it has informed the Chronicles design


% \subsection{Progressive and Optimistic Visualization}




% To deal with latency, chronicles adds the complexity of concurrent interactions while progressive/optimistic visualizations add the complexity of users working with, in addition to their data analysis, error bounds and .
% For users of the interactive system, working with the backend system overhead of online aggregation and approximate query processing in general is not so simple.  

% Moritz et al. developed a system, , that uses approximate query engine but allows users to.

% , and optimistic visualizations
% Aggregation (OLA) picks ever-growing samples and displays
% results to the user; when the analyst determines the visualization has tight-enough bounds, they can end the process. OLA
% computes aggregations and confidence intervals and returns
% them to the user.
% Hellerstein et al. [19] first suggested the idea; it has been adopted by the visualization community as a “progressive analytics” approach [13, 10, 36, 33, 39]. 

% Online aggregation processes ever-growing samples and , agarwal2013blinkdb}.
% While first proposed in the database community, the technique has been thoroughly explored by the visualization community as "progressive analytics".



% While powerful, progressive analytics adds additional mental overhead for 


% Sampling and ``progressive'' visualizations provide another avenue to achieve responsive access to approximate results~\cite{agarwal2013blinkdb, hellerstein1997online, fisher2012trust, zgraggen2016progressive}. However, 


% more relevant is 
% say that the mechanism of remembering used in Pangloss is often used as a mechanism to verify uncertain results. And say that what we find is other uses of history
% say that in the limit, Chronicles is a version of pangloss where each view is eagerly "remembered"?.
% also their remember is coupled with insights.
% also say that progressive optimisitic is superior in that they provide the user with some signal to work with. But we do not need to deal with the limitations of AQP, as well as without needing to change how the backend works, which might be appealing if the data already lives soemwhere and is expensive to migrate to a new processing system.


% This method lets analysts explore approximate results interactively, and provides a way to detect and recover from errors later.

% Much prior work in both the visualization and database community has been focused on reducing latency. 
% For example, using GPUs decreases compute time\cite{liu2013immens}, caching decreases latency for repeated interactions\cite{mohan2001caching}, prefetching decreases latency for predictable interactions\cite{battle2016, moritz2019falcon}, indexing decreases latency for specific interactions by pre-processing data \cite{gray1997data, lins2013nanocubes, tao2019kyrix}, and sampling decreases latency by providing estimated results\cite{hellerstein1997online,agarwal2013blinkdb}.

% An alternative to just improving system design is also to modify interaction design.  A body of work on \emph{progressive visualization} has integrated updated progressive results directly into the visualizations\cite{fisher2012trust, zgraggen2016progressive}.

% vis is important
% Our work takes motivation from prior findings on the negative effects of latency on interactive visualizations. Liu et al. observe that an additional delay of 500ms incurs high costs, reducing user activity, data set coverage, and the rate at which users draw generalizations and generate hypotheses\cite{liu2014effects}.

% past work
% The most direct solution to the issue of latency is to decrease it.  Researchers have developed a diverse range of techniques.
% how this relates to us
% Following the spirit of progressive visualizations, we also take the approach of making changes to the interaction design.  


% vis history
% \strikeg{Further, their design technique of encoding interaction order in another visual channel also informed our pilot designs of presenting past visual results as small multiples, which uses the position encoding channel.  The thumbnails in graphical histories helps us address the challenge of applying Chronicles to  dashboards, which takes up much space.
% However, we build off solutions from prior work to in the new problem domain of asynchronous interactive visualizations.} \remco{not necessary and feels a little blabbery}



==> chronicles-infovis-short-2020 (1)/makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> content/ack.tex <==
\add{\textbf{Acknowledgement}: Thanks to Larry Xu for early contributions, Aditya Parameswaran and the anonymous reviewers for their constructive comments. This material is based upon work supported by grants: NSF 1564049 1845638, 1564351, CCF-1730628, OAC-1940175, OAC-1939945, IIS-1452977, DGE-1855886, DARPA D3M (FA8750-17-2-0107), and DOE DE-SC0016934, as well as gifts from Alibaba, Amazon Web Services, Ant Financial, CapitalOne, Ericsson, Facebook, Futurewei, Google, Intel, Microsoft, Nvidia, Scotiabank, Splunk and VMware.}


==> content/scrap/design_scrap.tex <==

% show that presenting interaction histories do indeed facilitate users performing concurrent interactions when confronted with latency.  
% \remco{separate this sentence into two. First state what the generalized design is for? (e.g. ``We now present the generalized design for using interaction histories to XXXX.'' Then, the second sentence will be something like ``Named ``Chronicles'', this design requires three elements...''}: 

==> content/scrap/eval_scrap.tex <==
% \remco{need a conclusion section here... It's possible that 5.2 becomes the conclusion section? Not sure... but it feels weird to have a paper without one.}

% also just context
% History also proved useful outside of the context of concurrent interactions---it aided .  , all the participants clicked on a subset of past thumbnails, using the visuals as a base to recall their findings.


% The reason why not all interactions are concurrent can be explained by the analysis activities.  When participants had a specific question that compares across interactions, such as comparing between the fire counts by state across the years, they would concurrently specify their interactions. 

% A major limitation of Chronicle's approach is that it would only work for interactions that are not dependent on the previous interaction. Take Figure~\ref{fig:demo} as an example, if the analyst wishes to drill into states where the carrier United has the highest count of flights, then they necessarily have to wait until the data is loaded \jmh{for per-state carrier rankings} before they can proceed with the interaction \jmh{on the chosen states}.
% \jmh{Fig 1 is too small to understand at this level of detail.}
% However, as we have demonstrated in the pilot studies, there are basic tasks that involve interactions that are known ahead of time, such as finding a maximum, identifying if a threshold is crossed, identifying trends across interactions.  
% Furthermore, even for the aforementioned task where the next step is dependent on the previous, the user may benefit from having immediate access to the visualization state earlier in case they do not remember all the relevant values from some latency ago.

% The cases where one interaction may depend on a previous interaction state, as is the case of cross-filter, also uncovers possible extensions to the simple linear history we presented.  Future designs could iterate on a more complex tree-like thumbnail design that is shown on demand.

% Lastly, we need to conduct further user studies with more advanced tasks such as free form data exploration.  We also need to compare with progressive visualizations to get a better understanding of how the approaches compare.


% however, even if Chronicles cannot alleviate all the effects of delays, it is still valuable.



% talk about the different times when they do concurrent and when they don't---when they have a specific question to compare, they do, when they do not know what they are looking for, they need the result to inform their next steps.



% point toward literate computing

% Say that what we find with history corroborates with Moritz et al's finding "we might also group visualizations in the history by their broad tasks." --- say something along the lines of literate computing, the duality of seeing interactions as requests and in gneral artifacts that can be further worked with.





% talk about limitations, such as how we were not able to compare this against progressive visualizations.

==> content/scrap/future_scrap.tex <==

% that capturing interaction history in snapshots encourages users to make better use of waiting time. 

% To conclude, we discuss he last user study reveals opportunities for 



% open up the realization about history

% make it like a continuation of work that leverages interaction history
% By aiming to support concurrent interactions, we (re)discovered the power of history.  We could explore different affordances for the thumbnail design.

% TODO
% \jmh{I found this paragraph confusing and eventually unsatisfying once I unpacked it. It says that you have to wait on (cannot parallelize) data dependencies.  E.g. if you have two expressions $z = g(y)$ and $y = f(x)$, you have to wait for $y$ to be computed before you can execute $g(y)$. This is not a limitation of Chronicles per se. It's also weird to say "but there are cases where you don't have data dependencies." Of course there are. So question to you: if this is a "limitation", (a) what do you propose to do about it, and (b) how big of a limitation do you want to say it is? My personally feeling is that it's not a limitation of your work at all, it's an orthogonal fact about the real world that you can't do $g(f(x))$ before you do $f(x)$ and nobody would ever try to do so!!}


% Beyond assisting the analyst with tools against high latency, we hypothesize that the visual history may help analysts recall past insights and construct a narrative.
% In addition, the exact design of the history merits further design iterations---how long of the past should we show? Should we give users a way to store a view for future comparison manually?


==> content/scrap/related_scrap.tex <==

% Instead of progressively loading more data per interaction, we progressively load more results over a sequence of interactions. , but unlike Pangloss, interaction snapshots uses it as a stablizing frame of reference for asynchronous visualizations.
% The design space for asynchronous is orthogonal to progressive visualizations and face different trade offs.
% As a result, the challenges of the interface are also different. 

% Progressive visualization requires users to interpret uncertainty, whereas interaction snapshots requires users to specify interactions in advance of seeing previous results.
% diff
% Given that they lie in different design spaces, the two techniques are not mutually exclusive\,---\,design could compose Chronicles with progressive visualization to further enrich mechanisms against latency.


% Both progressive and optimistic visualizations need to work with sampling.  



% We now discuss in more detail how our approach relates to progressive and optimistic visualizations, both of which do make use of front-end design changes.

% We will not provide a detail discussion for backend methods to eliminate latency since our solution is concerned only with interaction design.  Our audience is those who have to work with some latencies, much like the audience of the progressive visualization research.  We will also discuss other research that make use of interaction history and how it has informed the Chronicles design


% \subsection{Progressive and Optimistic Visualization}




% To deal with latency, chronicles adds the complexity of concurrent interactions while progressive/optimistic visualizations add the complexity of users working with, in addition to their data analysis, error bounds and .
% For users of the interactive system, working with the backend system overhead of online aggregation and approximate query processing in general is not so simple.  

% Moritz et al. developed a system, , that uses approximate query engine but allows users to.

% , and optimistic visualizations
% Aggregation (OLA) picks ever-growing samples and displays
% results to the user; when the analyst determines the visualization has tight-enough bounds, they can end the process. OLA
% computes aggregations and confidence intervals and returns
% them to the user.
% Hellerstein et al. [19] first suggested the idea; it has been adopted by the visualization community as a “progressive analytics” approach [13, 10, 36, 33, 39]. 

% Online aggregation processes ever-growing samples and , agarwal2013blinkdb}.
% While first proposed in the database community, the technique has been thoroughly explored by the visualization community as "progressive analytics".



% While powerful, progressive analytics adds additional mental overhead for 


% Sampling and ``progressive'' visualizations provide another avenue to achieve responsive access to approximate results~\cite{agarwal2013blinkdb, hellerstein1997online, fisher2012trust, zgraggen2016progressive}. However, 


% more relevant is 
% say that the mechanism of remembering used in Pangloss is often used as a mechanism to verify uncertain results. And say that what we find is other uses of history
% say that in the limit, Chronicles is a version of pangloss where each view is eagerly "remembered"?.
% also their remember is coupled with insights.
% also say that progressive optimisitic is superior in that they provide the user with some signal to work with. But we do not need to deal with the limitations of AQP, as well as without needing to change how the backend works, which might be appealing if the data already lives soemwhere and is expensive to migrate to a new processing system.


% This method lets analysts explore approximate results interactively, and provides a way to detect and recover from errors later.

% Much prior work in both the visualization and database community has been focused on reducing latency. 
% For example, using GPUs decreases compute time\cite{liu2013immens}, caching decreases latency for repeated interactions\cite{mohan2001caching}, prefetching decreases latency for predictable interactions\cite{battle2016, moritz2019falcon}, indexing decreases latency for specific interactions by pre-processing data \cite{gray1997data, lins2013nanocubes, tao2019kyrix}, and sampling decreases latency by providing estimated results\cite{hellerstein1997online,agarwal2013blinkdb}.

% An alternative to just improving system design is also to modify interaction design.  A body of work on \emph{progressive visualization} has integrated updated progressive results directly into the visualizations\cite{fisher2012trust, zgraggen2016progressive}.

% vis is important
% Our work takes motivation from prior findings on the negative effects of latency on interactive visualizations. Liu et al. observe that an additional delay of 500ms incurs high costs, reducing user activity, data set coverage, and the rate at which users draw generalizations and generate hypotheses\cite{liu2014effects}.

% past work
% The most direct solution to the issue of latency is to decrease it.  Researchers have developed a diverse range of techniques.
% how this relates to us
% Following the spirit of progressive visualizations, we also take the approach of making changes to the interaction design.  


% vis history
% \strikeg{Further, their design technique of encoding interaction order in another visual channel also informed our pilot designs of presenting past visual results as small multiples, which uses the position encoding channel.  The thumbnails in graphical histories helps us address the challenge of applying Chronicles to  dashboards, which takes up much space.
% However, we build off solutions from prior work to in the new problem domain of asynchronous interactive visualizations.} \remco{not necessary and feels a little blabbery}



==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

